HalluPrism: When Multimodal Uncertainty Should Diagnose, Not Decide

Multimodal Large Language Models (MLLMs) can assign similar confidence to answers that fail for different reasons. We propose HalluPrism, a behavioral diagnostic that re-runs an answer after visual degradation, blank-image replacement, and grounding or relation checks. These targeted probes yield a signature over visual-perturbation sensitivity (V ), image-removal confidence retention (L), and grounding/relation-probe instability (A). Across 58K+ examples from four benchmarks and four MLLMs, image-removal confidence retention is most prevalent, while grounding/relation-probe instability better separates failure families. Only 18 of 48 source-target checks are diagonally aligned, so the coordinates should be interpreted jointly rather than as independent causal sources. With the dataset fixed, the joint signature improves failure-family AUROC from 0.634 to 0.769 on HallusionBench and from 0.707 to 0.817 on VizWiz, with smaller gains on POPE and VSR. In pooled XGBoost analysis, AUROC rises from 0.78 with scalar confidence to 0.95 with (V, L, A) and 0.97 when confidence is added. The same signature does not automatically improve correctness ranking. The three tested direct scalarizations can harm it. These results separate failure diagnosis from abstention scoring: multimodal uncertainty should characterize failure structure before it is used to decide whether to abstain or correct.

==> emnlp2023-latex/AIC/abstract.tex <==
\begin{abstract}
Multimodal Large Language Models (MLLMs) can assign similar confidence to answers that fail for different reasons. We propose \HalluPrism{}, a behavioral diagnostic that re-runs an answer after visual degradation, blank-image replacement, and grounding or relation checks. These targeted probes yield a signature over visual-perturbation sensitivity $(V)$, image-removal confidence retention $(L)$, and grounding/relation-probe instability $(A)$. Across 58K+ examples from four benchmarks and four MLLMs, image-removal confidence retention is most prevalent, while grounding/relation-probe instability better separates failure families. Only 18 of 48 source-target checks are diagonally aligned, so the coordinates should be interpreted jointly rather than as independent causal sources. With the dataset fixed, the joint signature improves failure-family AUROC from $0.634$ to $0.769$ on HallusionBench and from $0.707$ to $0.817$ on VizWiz, with smaller gains on POPE and VSR. In pooled XGBoost analysis, AUROC rises from $0.78$ with scalar confidence to $0.95$ with $(V,L,A)$ and $0.97$ when confidence is added. The same signature does not automatically improve correctness ranking. The three tested direct scalarizations can harm it. These results separate failure diagnosis from abstention scoring: multimodal uncertainty should characterize failure structure before it is used to decide whether to abstain or correct.
\end{abstract}


==> emnlp2023-latex/AIC/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

A visually grounded answer can be unsafe even when a Multimodal Large Language Model (MLLM) assigns high confidence to it. Consider a street-scene image where a traffic cone is to the right of a parked car, and the user asks: ``Is the traffic cone to the left of the car?'' The model may answer ``yes'' with high confidence. This single confident answer can hide several different risks. The cone may be small, blurred, or partly occluded, suggesting weak visual evidence. The model may answer ``yes'' even after the image is replaced with a blank canvas, pointing to language-prior reliance on the question alone. The model may also recognize both the cone and the car, while reversing the left-right relation, suggesting cross-modal binding failure. These risks require different responses - while a visually fragile answer may require abstention or visual re-grounding, a prior-driven answer may require anti-prior checking, and a relation error may require relation verification. Although scalar uncertainty can decide whether the model should answer, it does not say which of these responses is appropriate. Hence, in this paper, we argue that before uncertainty decides, it should \textit{diagnose} why the answer may fail.

Existing hallucination benchmarks already establish that multimodal errors are heterogeneous. They separate object hallucination, visual illusion, attribute error, spatial error, and answerability failure across different image-question regimes \citep{li2023evaluating,guan2024hallusionbench,wang2023amber,liu2023mmbench}. Confidence and calibration methods usually rank likely correctness or determine whether the model should abstain \citep{chow1970optimum,kadavath2022language,kuhn2023semantic,geng2023survey}. Recent MLLM uncertainty work moves closer to hallucination detection through evidential conflict, hidden-state reliability, and uncertain visual tokens \citep{huang2025evidentialconflict,mushtaq2025harmony,seo2025visualtokenuncertainty}. However, a diagnostic gap remains - i.e., \textit{whether the risk comes from weak visual evidence, language-prior reliance, or cross-modal binding}, apart from the scalar decision.

To address this, we propose \HalluPrism{}, a source-signature diagnostic for MLLM uncertainty. Given an image, a prompt, and a generated answer, \HalluPrism{} computes scalar confidence $c$ and a three-dimensional source signature $s(x)=(V,L,A)$. The coordinates measure visual fragility $(V)$, language-prior reliance $(L)$, and cross-modal alignment instability $(A)$ through controlled perturbation probes. In the traffic-cone example, $V$ increases when blur, crop, darkness, or noise changes the answer or its confidence. $L$ increases when the answer survives after the image is replaced by a blank image. $A$ increases when grounding or relation perturbations expose instability in the left-right binding. 
% This follows the behavioral-testing view that controlled input changes can expose brittle decision boundaries \citep{ribeiro2020checklist,gardner2020contrastsets,kaushik2020counterfactually}. 
$s(x)$ is a perturbation-response profile and not a decomposition of hidden mechanisms inside the model. Hence, a high $L$ does not prove that the model never used the image. Similarly, high $V$ or $A$ records sensitivity under visual or alignment pressure rather than isolating a single internal failure cause. In other words, \HalluPrism{} helps to diagnose and route failures as a \textit{joint} behavioral signature instead of assigning each error to one clean causal source.

% We find across $58{,}440$ model-dataset examples that source-aware uncertainty is more useful for diagnosis than for naive scalar confidence replacement. Language-prior reliance is nearly universal. The raw dominant source is language-prior for $99.7\%$ of samples. However, prevalence is not diagnostic value. In tree-based failure-family prediction, alignment is the strongest feature in the pooled model, with importance $0.504$. Controlled interventions explain this distinction. If $V$, $L$, and $A$ were clean source labels, visual-ruined inputs would mainly affect $V$, language-ruined inputs would mainly affect $L$, and alignment-ruined inputs would mainly affect $A$. We find that this diagonal pattern is rare. Only $7$ of $48$ intervention checks satisfy diagonal dominance, and visual-ruined inputs pass in $0$ of $16$ settings. \HalluPrism{} therefore treats $(V,L,A)$ as a joint source signature rather than a one-source explanation. 
% The joint signature is strongly diagnostic. In pooled failure-family prediction, scalar confidence reaches AUROC $0.781$ with XGBoost. The source signature reaches $0.954$, and the combined representation reaches $0.971$. The same source information behaves differently when forced into a single abstention score. Weighted, geometric, and max-penalty scalarizations underperform scalar confidence for abstention across the four model families. For Qwen3-VL, scalar confidence reaches AUROC $0.809$, while the best source-aware scalarization reaches $0.732$. This is the source-aware confidence trap. The signal that explains failure family can damage the answer-versus-abstain ranking. We also test whether source signatures can route interventions. On Qwen3-VL/Visual Spatial Reasoning (VSR), generic prompting reduces accuracy from $87.4\%$ to $76.2\%$ and breaks $15.5\%$ of originally correct predictions. Matched routing maintains $87.6\%$ accuracy and reduces the break rate to $2.7\%$.

Across $58{,}440$ model-dataset examples, source-aware uncertainty is more useful for diagnosis than for naive scalar confidence replacement. Language-prior reliance is nearly universal, with language-prior as the raw dominant source for $99.7\%$ of samples. However, prevalence is not diagnostic value. Alignment is the strongest pooled feature in tree-based failure-family prediction, with importance $0.504$. Controlled interventions explain this gap. If $V$, $L$, and $A$ were clean source labels, visual-, language-, and alignment-ruined inputs would mainly affect their corresponding coordinates. Only $7$ of $48$ intervention checks satisfy this diagonal pattern, and visual-ruined inputs pass in $0$ of $16$ settings. \HalluPrism{} therefore treats $(V,L,A)$ as a joint source signature rather than a one-source explanation.
The joint signature is strongly diagnostic. With XGBoost, pooled failure-family AUROC improves from $0.781$ with scalar confidence to $0.954$ with $(V,L,A)$, and to $0.971$ with the combined representation. The same signal weakens abstention when forced into one score. Weighted, geometric, and max-penalty scalarizations underperform scalar confidence across all four model families. For Qwen3-VL, AUROC drops from $0.809$ to $0.732$. This source-aware confidence trap shows that a signal useful for failure typing can damage answer-versus-abstain ranking. Source signatures can still help routing. On Qwen3-VL/Visual Spatial Reasoning (VSR), generic prompting reduces accuracy from $87.4\%$ to $76.2\%$ and breaks $15.5\%$ of originally correct predictions, while matched routing maintains $87.6\%$ accuracy and reduces break rate to $2.7\%$.

\textbf{Contributions}. (i) We identify the source-aware confidence trap, where naive scalarization weakens abstention despite strong diagnostic value. (ii) We propose \HalluPrism{} as a perturbation-response signature over visual fragility, language-prior reliance, and cross-modal alignment instability. (iii) We show that controlled probes reveal interventional entanglement rather than clean source separability. (iv) We show that source signatures support bounded diagnostic and routing use. They add information beyond dataset and model identity in controlled failure-family diagnosis, and they reduce harmful breakage from generic interventions in selected high-risk settings.


==> emnlp2023-latex/AIC/related-work.tex <==
\section{Related Work}
\label{sec:related_work}

\paragraph{Multimodal Hallucination Evaluation.} Vision-language hallucination work shows that multimodal errors are not a single phenomenon. Captioning and Visual Question Answering (VQA) studies connect object hallucination and apparent visual reasoning to language priors and weak grounding \citep{rohrbach2018object,goyal2017making}. MLLM benchmarks make this heterogeneity more explicit. While POPE measures object-presence hallucination \citep{li2023evaluating}, HallusionBench targets entangled language hallucination and visual illusion \citep{guan2024hallusionbench}. AMBER covers existence, attribute, and relation errors \citep{wang2023amber}, while broader suites such as MME and MMBench show divergence across perception, reasoning, and instruction following \citep{fu2023mme,liu2023mmbench}. \HalluPrism{} changes the unit of analysis. Instead of assigning only a benchmark score or hallucination label, it measures a behavioral source signature over visual fragility, language-prior reliance, and cross-modal alignment instability.

\paragraph{Uncertainty, Calibration, and Selective Prediction.} Classical reject-option and selective-classification work frames uncertainty as a decision problem. A model should answer when risk is low and abstain otherwise \citep{chow1970optimum,geifman2017selective,geifman2019selectivenet}. Calibration asks whether confidence values match empirical correctness \citep{guo2017calibration}. Language-model uncertainty extends this question to generated text through self-estimation, token-probability aggregation, or semantic equivalence classes \citep{kadavath2022language,kuhn2023semantic,geng2023survey}. Black-box hallucination detection methods such as SelfCheckGPT use sample inconsistency as a factuality signal \citep{manakul2023selfcheckgpt}. In multimodal settings, selective answering and unnecessary-abstention reduction have been studied for visual reasoning and VQA \citep{eisenschlos2024selectively,srinivasan2024selective}. Recent MLLM uncertainty methods move closer to hallucination diagnosis through evidential conflict, hidden-state reliability, and visual-token epistemic uncertainty \citep{huang2025evidentialconflict,mushtaq2025harmony,seo2025visualtokenuncertainty}. In contrast to giving a single correctness-ranking score, \HalluPrism{} treats uncertainty as a source signature for diagnosis and routing.

\paragraph{Behavioral Probing, Attribution, and Source Entanglement.} Behavioral testing studies model behavior through controlled input changes. CheckList exposes capability-specific failures \citep{ribeiro2020checklist}. Contrast sets and counterfactually augmented data reveal brittle behavior under small edits \citep{gardner2020contrastsets,kaushik2020counterfactually}. Attribution methods ask a more internal question, for example by localizing visual regions with Grad-CAM \citep{selvaraju2017gradcam} or analyzing attention and attention flow \citep{jain2019attention,abnar2020quantifying}. Multimodal hallucination work also studies attention directly, such as DAMRO's analysis of image-token attention and background outliers \citep{gong2024damro}. \HalluPrism{} follows the behavioral-testing view rather than the internal-attribution view. It asks how the output changes when we pressure the visual channel, the language-only channel, or the cross-modal binding channel. 
% Off-target responses under these probes are retained because they show that source coordinates should be read jointly rather than as independent causal labels.

\paragraph{Hallucination Mitigation and Intervention Routing.} Many mitigation methods apply a fixed correction rule during decoding or after generation. Visual Contrastive Decoding contrasts predictions under original and distorted visual inputs \citep{leng2023mitigating}. OPERA penalizes hallucination-prone decoding patterns \citep{huang2023opera}. M3ID amplifies image-grounded information against language priors \citep{favero2024multimodal}. Woodpecker and Volcano use post-hoc correction or self-feedback revision \citep{yin2023woodpecker,lee2023volcano}. Recent inference-time methods refine this direction through inter-modality calibration, attention calibration, and visual-aware sparsification \citep{li2025imccd,fazli2025caac,zhuang2025vasparse}. \HalluPrism{} is positioned one step earlier. It first profiles failure behavior and then asks whether the intervention should be matched to the measured source signature. This is why we evaluate both fix rate and break rate. A generic intervention can repair some incorrect answers while damaging correct multimodal predictions.


==> emnlp2023-latex/Figures/Fig-HalluPrism_Detailed.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.65\textwidth]{emnlp2023-latex/Figures/HalluPrism Pipeline.png}
    \caption{Overview of the \HalluPrism{} perturbation-response source-signature protocol. The scores are behavioral probes, not a causal decomposition. Detailed figure in }
    \label{fig:halluprism_detailed_fig}
\end{figure*}

==> emnlp2023-latex/Methodology/HalluPrism-reframed.tex <==
% \input{emnlp2023-latex/Figures/Fig - HalluPrism}

\section{Methodology}
\label{sec:halluprism}

We study multimodal uncertainty as a \textit{{pre}-decision} diagnostic object. The goal is not to construct a better scalar abstention score, but to test whether a prediction carries a behavioral source signature that can diagnose failure family and route correction without assuming clean causal separability. \textit{All cited Propositions, Theorems, Corollaries, and Definitions in this section are given in the Theoretical Analysis section of Appendix \ref{app:formal_support}}.
% The formal results in Appendix~\ref{app:formal_support} support this role separation. 
% To illustrate, suppose the input image contains a traffic cone to the right of a parked car, and the prompt asks whether the cone is to the left of the car. The generated answer may be ``yes'' with high scalar confidence. HalluPrism does not ask only whether this answer is likely to be correct. It asks how the answer behaves when visual evidence is degraded, when the image is removed, and when the relation is explicitly stressed. These three probes define the source signature used below.

% \paragraph{Prediction, Confidence, and Source Signatures}
% \label{subsec:prediction_confidence_source}

% Let $x=(I,q)$ denote an image ($I$)-prompt ($q$) input, and let a Multimodal Large Language Model (MLLM) $M$ generate $\hat{y}=M(I,q)$. Each example has a reference answer $y$ or an answerability label. We write correctness after task-specific answer normalization as:
% \begin{equation}
% \begin{split}
% & z(x,M)=\mathbf{1}[\mathrm{norm}(\hat{y})=\mathrm{norm}(y)].
% \end{split}
% \label{eq:correctness}
% \end{equation}
% Incorrect outputs receive a failure-family label $f(x,M)\in\mathcal{F}$, including \texttt{object-hallucination}, \texttt{spatial/relation-error}, \texttt{attribute-error}, and \texttt{answerability-failure}. Correct outputs receive \texttt{None}. The label describes the task-level failure pattern. 
% A scalar confidence estimator maps an input-output instance to $c(x,M)\in[0,1]$. For an answer $\hat{y}=(t_1,\ldots,t_N)$, we use length-normalized answer probability:
% \begin{equation}
% \begin{split}
% & c(\hat{y}\mid I,q)=\exp\left(\frac{1}{N}\sum_{i=1}^{N}\log p(t_i\mid t_{<i},I,q)\right).
% \end{split}
% \label{eq:scalar_confidence}
% \end{equation}
% For binary and true/false tasks, we normalize the generated answer to the task label space before scoring correctness. For VizWiz-VQA, we use dataset-specific answer normalization and answer-level token confidence. This scalar score ranks correctness, although it does not identify whether an answer is visually fragile, language-prior driven, or cross-modally misaligned. This scalar non-identifiability is formalized in Proposition~\ref{prop:scalar_nonidentifiability}.
% We define a source signature as:
% \begin{equation}
% \begin{split}
% & s(x,M)=(V(x,M),L(x,M),A(x,M)),\\
% & s(x,M)\in[0,1]^3.
% \end{split}
% \label{eq:source_signature}
% \end{equation}
% The coordinate $V$ measures visual fragility, $L$ measures language-prior reliance, and $A$ measures cross-modal alignment instability. These values are behavioral signals induced by controlled probes. They are not assumed to recover independent hidden mechanisms. A source signature can still be useful when scores are entangled because failure families may occupy different regions of the joint $(V,L,A)$ space.


\paragraph{Prediction and Source Signatures.}
\label{subsec:prediction_source_signatures}
Consider the street-scene example of an image $I$ containing a traffic cone to the right of a parked car, and a prompt $q$ asks whether the cone is to the left of the car. If an MLLM $M$ answers ``\textit{yes}'' to the input $x=(I,q)$ (denoted $\hat{y}$) while the reference answer (denoted $y$) is ``\textit{no}'', the output is incorrect\footnote{We use answer normalization before this comparison, to map surface variants such as ``yes'', ``Yes.'', or ``yes, it is'' to the same canonical task label.}. 
Although this correctness label is useful for abstention, it does not explain why the answer failed. 
% The same wrong answer may be visually fragile if the cone is hard to see, language-prior driven if the answer survives without the image, or alignment-sensitive if the model recognizes both objects but reverses the left-right relation.
In our settings, each input example has either a reference answer $y$, such as \texttt{yes}, \texttt{no}, an object label, or an attribute label, or an answerability label, such as \texttt{answerable} or \texttt{unanswerable}, indicating whether the image contains enough information to answer the prompt. We write correctness as $z(x,M)=\mathbf{1}[\mathrm{norm}(\hat{y})=\mathrm{norm}(y)]$.
% \begin{equation}
% \begin{split}
% & z(x,M)=\mathbf{1}[\mathrm{norm}(\hat{y})=\mathrm{norm}(y)].
% \end{split}
% \label{eq:correctness}
% \end{equation}
Incorrect outputs receive a failure-family label $f(x,M)\in\mathcal{F}$, including \texttt{object-hallucination}, \texttt{spatial/relation-error}, \texttt{attribute-error}, and \texttt{answerability-failure}.
A scalar confidence estimator maps the input-output instance to $c(x,M)\in[0,1]$. A length-normalized tokenized answer $\hat{y}=(t_1,\ldots,t_N)$ has confidence probability:
\begin{equation}
\begin{split}
& c(\hat{y}\mid I,q)=\exp\left(\frac{1}{N}\sum_{i=1}^{N}\log p(t_i\mid t_{<i},I,q)\right).
\end{split}
\label{eq:scalar_confidence}
\end{equation}
% For binary and true/false tasks, we first map the generated answer to the task label space. For example, answers such as \texttt{yes}, \texttt{Yes.}, and \texttt{yes, it is} are treated as the same \texttt{yes} label before correctness is computed. 
For answerability-focused datasets, we apply the dataset-specific normalization rule and use the model's token-level probability for the normalized answer as confidence. 
% This gives a scalar score for ranking likely correctness. However, the score only says how confident the model is in the final answer. It does not say whether the answer depends on weak visual evidence, survives as a language prior without the image, or fails because the image-text relation is misbound. This scalar non-identifiability is formalized in Proposition~\ref{prop:scalar_nonidentifiability}.
This gives a scalar score for ranking likely correctness. However, the score only indicates how confident the model is in the final answer. It does not say whether the answer depends on weak visual evidence, survives as a language prior without the image, or fails because the image-text relation is misbound. \textit{Hence, scalar confidence is a correctness-ranking surrogate, not a grounded reliability certificate}. This scalar non-identifiability is formalized in Proposition~\ref{prop:scalar_nonidentifiability}.
We attach a $[0,1]$-bounded source signature to the same prediction:
\begin{equation}
\begin{split}
& s(x,M)=(V(x,M),L(x,M),A(x,M))
\end{split}
\label{eq:source_signature}
\end{equation}
$V$ measures visual fragility, $L$ measures language-prior reliance, and $A$ measures cross-modal alignment instability. They are behavioral signals induced by controlled probes, as discussed in the next section. Although they do not recover hidden mechanisms, a source signature is useful under entanglement because failure families may occupy different regions of the joint $(V,L,A)$ space.




% \paragraph{Perturbation Probes}
% \label{subsec:perturbation_probes}

% Each source score compares the clean answer with answers produced under controlled probes. Let $\mathrm{flip}(\hat{y},\tilde{y})$ be $1$ when the perturbed answer differs from the clean answer after normalization and $0$ otherwise. Let $\Delta c(\hat{y},\tilde{y})=|c(\hat{y})-c(\tilde{y})|$. Answer flips capture discrete instability. Confidence shifts capture softer changes when the final answer remains unchanged.
% The visual score $V$ measures sensitivity to degraded visual evidence. In our example, this tests whether the cone-car answer changes when the cone becomes blurred, cropped out, darkened, or corrupted by visual noise. We construct $K=4$ image variants using Gaussian blur, center crop, brightness reduction, and Gaussian noise, while keeping the prompt fixed.
% % The visual score $V$ measures sensitivity to degraded visual evidence. We construct $K=4$ image variants using Gaussian blur, center crop, brightness reduction, and Gaussian noise, while keeping the prompt fixed. In our example, this tests whether the cone-car answer changes when the cone becomes blurred, cropped out, darkened, or corrupted by visual noise.
% For the $k$-th perturbed answer $\tilde{y}^{v}_{k}$, we define:
% \begin{equation}
% \begin{split}
% & V=0.6\cdot\frac{1}{K}\sum_{k=1}^{K}\mathrm{flip}(\hat{y},\tilde{y}^{v}_{k}) \\
% & \qquad +0.4\cdot\min\left(2\cdot\frac{1}{K}\sum_{k=1}^{K}\Delta c(\hat{y},\tilde{y}^{v}_{k}),1\right).
% \end{split}
% \label{eq:visual_score}
% \end{equation}
% The larger flip weight makes changed answers the primary signal of visual fragility.
% The language-prior score $L$ measures answer survival when visual evidence is removed. 
% This tests whether the model still gives the same left-right answer about the traffic cone and the parked car after both objects are removed by replacing the image with a blank canvas.
% We replace the image with a uniform blank image $I_{\mathrm{blank}}$ and keep the same prompt. Let $\tilde{y}^{\ell}$ be the blank-image answer. We define:
% \begin{equation}
% \begin{split}
% & L=\mathbf{1}[\mathrm{match}(\hat{y},\tilde{y}^{\ell})]\cdot\min\left(\frac{c(\tilde{y}^{\ell})}{c(\hat{y})+\epsilon},1\right).
% \end{split}
% \label{eq:language_score}
% \end{equation}
% A high value indicates that the same answer persists with similar confidence without the original image. It is a behavioral marker, not a claim that the model ignores the image in every case.
% The alignment score $A$ measures sensitivity to cross-modal binding pressure. 
% This tests whether the model keeps the same answer when the left-right relation between the traffic cone and the parked car is re-queried or swapped.
% We use a grounding prompt for all datasets and add a negation or relation-swap probe when the task structure allows it. VSR provides direct spatial perturbations through terms such as left, right, above, below, in front of, and behind. Let $\tilde{y}^{a}_{\mathrm{ground}}$ be the grounding-prompt answer and $\tilde{y}^{a}_{\mathrm{rel}}$ the relation-perturbed answer when available. We define:
% \begin{equation}
% \begin{split}
% & P_g=0.5\cdot\mathrm{flip}(\hat{y},\tilde{y}^{a}_{\mathrm{ground}})\\
% & \qquad +\min(\Delta c(\hat{y},\tilde{y}^{a}_{\mathrm{ground}}),0.5), \\
% & P_r=\mathbf{1}[\mathrm{available}]\cdot\mathbf{1}[\mathrm{relation\ inconsistent}], \\
% & A=\begin{cases}
% \min(0.4P_g+0.6P_r,1), & \mathrm{if\ available},\\
% \min(P_g,1), & \mathrm{otherwise}.
% \end{cases}
% \end{split}
% \label{eq:alignment_score}
% \end{equation}
% The relation term receives larger weight when available because it directly tests whether the answer changes consistently with the controlled relation perturbation.


\paragraph{Perturbation Probes.}
\label{subsec:perturbation_probes}
We measure each source score by asking how the same prediction behaves under controlled input pressure. The clean answer $\hat{y}$ is the baseline. A probe changes one part of the input and produces a perturbed answer $\tilde{y}$. We use \textit{perturbation} for the local probes used to compute $V$, $L$, and $A$. We use \textit{ruined condition} for the stronger source-targeting condition used later in the diagonal-dominance test, where the full source signature is recomputed after targeting one channel.
% We measure each source score by asking how the same prediction behaves under controlled input pressure. The clean answer $\hat{y}$ is the baseline. A probe changes one part of the input and produces a perturbed answer $\tilde{y}$. 
% We compare $\hat{y}$ and $\tilde{y}$ using answer change and confidence change. Let $\mathrm{flip}(\hat{y},\tilde{y})$ be $1$ when the perturbed answer differs from the clean answer and $0$ otherwise. Let $\Delta c(\hat{y},\tilde{y})=|c(\hat{y})-c(\tilde{y})|$. Answer flips capture discrete instability. Confidence shifts capture softer changes when the final answer remains unchanged. The \textbf{visual score} $V$ measures sensitivity to degraded visual evidence. In our example, this tests whether the cone-car answer changes when the cone becomes blurred, cropped out, darkened, or corrupted by visual noise. We construct 4 image variants using Gaussian blur ($\sigma\!=\!15$), center crop (50\% per dimension, resized back), brightness reduction (30\% of original), and Gaussian noise ($\mu\!=\!0, \sigma\!=\!25$), while keeping the prompt fixed. 
We compare $\hat{y}$ and $\tilde{y}$ using answer and confidence changes. Let $\mathrm{flip}(\hat{y},\tilde{y})=1$ if the perturbed answer differs from the clean answer, and $0$ otherwise. Let $\Delta c(\hat{y},\tilde{y})=|c(\hat{y})-c(\tilde{y})|$. Flips capture discrete instability, while confidence shifts capture softer changes when the answer is unchanged. The \textbf{visual score} $V$ measures sensitivity to degraded visual evidence. In the cone-car example, this tests whether the answer changes when the cone is blurred, cropped, darkened, or corrupted by noise. We construct four image variants while keeping the prompt fixed: Gaussian blur ($\sigma\!=\!15$), center crop ($50\%$ per dim., resized back), $30\%$ brightness reduction, and Gaussian noise ($\mu\!=\!0,\sigma\!=\!25$).
For $k$-th perturbed answer $\tilde{y}^{v}_{k}$:
\begin{equation}
\begin{split}
& V=0.6\cdot\frac{1}{K}\sum_{k=1}^{K=4}\mathrm{flip}(\hat{y},\tilde{y}^{v}_{k}) \\
& \qquad +0.4\cdot\min\left(2\cdot\frac{1}{K}\sum_{k=1}^{K}\Delta c(\hat{y},\tilde{y}^{v}_{k}),1\right).
\end{split}
\label{eq:visual_score}
\end{equation}
The larger flip weight makes changed answers the primary signal of visual fragility.
The \textbf{language-prior score} $L$ measures answer survival when visual evidence is removed. This tests whether the model still gives the same left-right answer about the traffic cone and the parked car after both objects are removed by replacing the image with a blank canvas. We replace the image with a uniform blank image $I_{\mathrm{blank}}$ and keep the same prompt. Let $\tilde{y}^{\ell}$ be the blank-image answer. We define:
\begin{equation}
\begin{split}
& L=\mathbf{1}[\mathrm{match}(\hat{y},\tilde{y}^{\ell})]\cdot\min\left(\frac{c(\tilde{y}^{\ell})}{c(\hat{y})+\epsilon},1\right).
\end{split}
\label{eq:language_score}
\end{equation}
% Here $\mathrm{match}(\hat{y},\tilde{y}^{\ell})$ checks equality after the same answer-normalization rule used for correctness. 
% A high $L$ means that the same answer persists with similar confidence without the original image. As discussed earlier, it is a behavioral marker and does not imply that the model ignores the image in every case.
% The \textbf{alignment score} $A$ measures sensitivity to cross-modal binding pressure. This tests whether the model keeps the same answer when the left-right relation between the traffic cone and the parked car is re-queried or swapped. We use two alignment probes. The first probe is available for all datasets. It asks the model to ground the answer by re-checking the relevant visual evidence. The second probe is used only when the task has an explicit relation that can be perturbed. Visual Spatial Reasoning (VSR) is the clearest such case, because its prompts contain spatial relations such as \textit{left}, \textit{right}, \textit{above}, \textit{below}, \textit{in front of}, and \textit{behind}. In the cone-car example, if the clean prompt asks whether the cone is to the left of the car, the relation-swapped prompt asks the corresponding right-of question. A relation-sensitive model should not preserve the same normalized answer under both prompts.
% Let $\tilde{y}^{a}_{\mathrm{ground}}$ be the grounding-prompt answer. Let $\tilde{y}^{a}_{\mathrm{rel}}$ be the relation-swapped answer when such a swap is available. The grounding penalty $P_g$ captures instability under visual re-checking. The relation penalty $P_r$ captures a failure to change the answer under a controlled relation swap where the expected answer should change.
A high $L$ means that the same answer persists with similar confidence without the original image. It is a behavioral marker and does not imply that the model ignores the image in every case. The \textbf{alignment score} $A$ measures sensitivity to cross-modal binding pressure. It tests whether the answer remains stable when the relevant image-text relation is re-queried or swapped. We use two alignment probes. The first is available for all datasets and asks the model to re-check the relevant visual evidence. The second is used only when the task has an explicit perturbable relation. Visual Spatial Reasoning (VSR) is the clearest case, because its prompts contain spatial relations such as \textit{left}, \textit{right}, \textit{above}, \textit{below}, \textit{in front of}, and \textit{behind}. In the cone-car example, if the clean prompt asks whether the cone is to the left of the car, the relation-swapped prompt asks the corresponding right-of question. A relation-sensitive model should not preserve the same normalized answer under both prompts. Let $\tilde{y}^{a}_{\mathrm{ground}}$ be the grounding-prompt answer, and let $\tilde{y}^{a}_{\mathrm{rel}}$ be the relation-swapped answer when available. The grounding penalty $P_g$ captures instability under visual re-checking, while the relation penalty $P_r$ captures failure to change under a controlled relation swap where the expected answer should change.
We define:
\begin{equation}
\begin{split}
& P_g=0.5\cdot\mathrm{flip}(\hat{y},\tilde{y}^{a}_{\mathrm{ground}})\\
& \qquad +\min(\Delta c(\hat{y},\tilde{y}^{a}_{\mathrm{ground}}),0.5), \\
& P_r=\mathbf{1}[\mathrm{available}]\cdot
\mathbf{1}[\mathrm{norm}(\tilde{y}^{a}_{\mathrm{rel}})=\mathrm{norm}(\hat{y})], \\
& A=\begin{cases}
\min(0.4P_g+0.6P_r,1), & \mathrm{if\ available},\\
\min(P_g,1), & \mathrm{otherwise}.
\end{cases}
\end{split}
\label{eq:alignment_score}
\end{equation}
$A$ increases when $P_r$ is present because it directly tests whether the model preserves an answer under a controlled relation swap where the expected answer should change.




\paragraph{Interpreting And Using Source Signatures.}
\label{subsec:diagnosis_abstention_routing}
Once the probes produce $(V,L,A)$, we use the vector for three linked questions. First, \textit{which coordinate is largest}? Second, \textit{does a targeted intervention mainly move its intended coordinate}? Third, \textit{does the full signature help diagnosis, abstention, or routing}? These questions must be separated because a large coordinate is not a causal assignment. If $L$ is largest, the prediction is counted as language-prior dominant because the answer strongly survives blank-image probing. In the cone-car example, the model may still give the same answer without the image and also fail because it reverses the left-right relation. Hence, \textbf{raw dominance} is only a counting device. It assigns each prediction to the largest of $V$, $L$, and $A$ as $s^{*}_{\mathrm{raw}}(x,M)=\arg\max_{Q\in\{V,L,A\}} Q(x,M)$.
% \begin{equation}
% \begin{split}
% & s^{*}_{\mathrm{raw}}(x,M)=\arg\max_{Q\in\{V,L,A\}} Q(x,M).
% \end{split}
% \label{eq:raw_dominance}
% \end{equation}
Because one coordinate can saturate, we also use a within-setting \textbf{normalized dominant} source $s^{*}_{\mathrm{norm}}(x,M)=\arg\max_{Q\in\{V,L,A\}} z_Q(x,M)$, where $z_Q(x,M)=(Q(x,M)-\mu_Q)/(\sigma_Q+\epsilon)$. We use normalized dominance for intervention routing. It prevents a nearly saturated coordinate, say $L$, from dominating every routing decision.

% We next test whether the source scores behave as separable labels. In the cone-car example, a visual intervention should mainly change $V$ if the scores are separable, while a left-right relation intervention should mainly change $A$. Let $T_V$, $T_L$, and $T_A$ denote controlled perturbations that target visual evidence, language-prior reliance, and alignment. For target $R$ and coordinate $Q\in\{V,L,A\}$, define $\Delta_{R,Q}(x,M)=Q(T_R(x),M)-Q(x,M)$. A cleanly separable signature would satisfy:
% \begin{equation}
% \begin{split}
% & \Delta_{R,R}(x,M)>\max_{Q\neq R}\Delta_{R,Q}(x,M).
% \end{split}
% \label{eq:diagonal_condition_main}
% \end{equation}
% We measure whether this property holds rather than assuming it. Definition~\ref{def:diagonal_separability} states the probe-level condition. Proposition~\ref{prop:probe_entanglement} establishes that off-target responses prevent a one-to-one interpretation of an intervention as affecting only its intended source.

We next test whether the source scores behave as separable labels. In the cone-car example, a visual intervention should produce the largest absolute change in $V$ if the scores are separable, while a left-right relation intervention should produce the largest absolute change in $A$. Let $\mathcal{T}_V$, $\mathcal{T}_L$, and $\mathcal{T}_A$ denote the visual-ruined, language-ruined, and alignment-ruined conditions used for this test. These ruined conditions are stronger than the local perturbations used to compute the source scores. For target $R$ and coordinate $Q\in\{V,L,A\}$, define:
\begin{equation}
\begin{split}
& \Delta_{R,Q}(x,M)=Q(\mathcal{T}_R(x),M)-Q(x,M).
\end{split}
\label{eq:intervention_response_main}
\end{equation}
A cleanly separable signature would satisfy magnitude-based diagonal dominance:
\begin{equation}
\begin{split}
& |\Delta_{R,R}(x,M)|>\max_{Q\neq R}|\Delta_{R,Q}(x,M)|.
\end{split}
\label{eq:diagonal_condition_main}
\end{equation}
We measure whether this property holds. Definition~\ref{def:diagonal_separability} states the separability condition and 
% Proposition~\ref{prop:probe_entanglement} establishes that an off-target response with comparable or larger magnitude prevents a one-to-one interpretation of an intervention as affecting only its intended source.
Proposition~\ref{prop:probe_entanglement} proves this limitation: \textit{if one source intervention leads to a greater than or equal change in any other source score, then it cannot be interpreted as source-specific}.


We then evaluate three uses of source signatures: (i) failure-family diagnosis, (ii) abstention scalarization, and (iii) intervention routing. These uses test different claims. Diagnosis asks whether the signature explains the kind of error. Abstention scalarization asks whether the signature should be collapsed into one answer-versus-abstain score. Routing asks whether the signature helps choose a safer correction path. In failure-family diagnosis, we ask whether $s(x,M)$ predicts $f(x,M)$ better than scalar confidence alone. The role separation follows from Proposition~\ref{prop:diagnosis_not_abstention} and Theorem~\ref{thm:role_separation}: source signatures can help failure-family prediction even when scalar confidence remains sufficient for Bayes-optimal abstention. In abstention, we ask whether a scalarized source-aware score $\tilde{c}(x,M)=g(c,V,L,A)$ improves correctness ranking. Proposition~\ref{prop:pairwise_inversion} and Corollary~\ref{cor:saturation_ranking} prove why source penalties can reverse useful confidence orderings, especially when one coordinate is saturated. In routing, a policy maps $s(x,M)$ to no intervention, visual re-grounding, anti-prior prompting, or relation checking. Proposition~\ref{prop:routing_decomposition} and Corollary~\ref{cor:break_rate_importance} explain why fix rate and break rate must be reported with accuracy.
For abstention, we test three source-aware scalarizations:
\begin{equation}
\begin{split}
& c_{\max}=c\cdot(1-\max(V,L,A)),\\
& c_w=c\cdot(1-0.3V-0.3L-0.4A),\\
& c_{\mathrm{geo}}=c\cdot((1-V)(1-L)(1-A))^{1/3}.
\end{split}
\label{eq:scalarizations}
\end{equation}
For intervention routing, a generic baseline applies the same reasoning prompt to every input. The matched policy maps $s^{*}_{\mathrm{norm}}(x,M)$ to visual re-grounding, anti-prior prompting, or relation checking. For example, an alignment-dominant cone-car prediction is routed to relation checking rather than to a generic reasoning prompt. We report accuracy, fix rate, and break rate:
\begin{equation}
\begin{split}
& \mathrm{Fix}=\frac{\#\{\mathrm{incorrect}\rightarrow\mathrm{correct}\}}{\#\{\mathrm{incorrect}\}},\\
& \mathrm{Break}=\frac{\#\{\mathrm{correct}\rightarrow\mathrm{incorrect}\}}{\#\{\mathrm{correct}\}}.
\end{split}
\label{eq:fix_break_main}
\end{equation}
We do a clean forward pass, four visual perturbation passes, one blank-image pass, and one or two alignment passes, depending on whether relation perturbation is available, without retraining.




==> emnlp2023-latex/Results/results-reframed.tex <==
\input{emnlp2023-latex/Tables/Tab-Source-profile-and-entanglement}

\input{emnlp2023-latex/Tables/Tab-Diagnosis-and-importance}

\input{emnlp2023-latex/Tables/Tab-Decision-behavior}

\section{Results}
\label{sec:results}

We evaluate $(V,L,A)$ for failure typing and matched correction, not as a direct scalar confidence replacement.

\paragraph{Prevalence is not Diagnostic Value.}
\label{subsec:source_profiles}
We observe from Table~\ref{tab:source_entanglement_main} that $L$ is high across settings, with means from $0.91$ to $1$ and language-prior match from $37.6\%$ to $96.5\%$. VizWiz has the highest visual scores ($0.19$ to $0.30$), while Gemma 4/VSR and Qwen3-VL/VSR have the highest alignment scores ($0.68$ and $0.61$). Raw dominance is almost entirely language-prior: $58{,}287/58{,}440$ samples are $L$-dominant, versus $151$ for $A$ and $2$ for $V$. We therefore treat prevalence as saturation, not diagnostic value.

\paragraph{Interventions Expose Entanglement.}
\label{subsec:entanglement}
We test whether visual-ruined, language-ruined, and alignment-ruined inputs isolate their intended coordinate under Definition~\ref{def:diagonal_separability}. We observe from Table~\ref{tab:source_entanglement_main} that Qwen3-VL/HallusionBench separates signed and magnitude responses: visual ruin decreases $V$ by $0.09$ with small $L/A$ changes, while language ruin decreases $L$ by $0.09$ and increases $A$ by $0.18$. Overall, only $18/48$ checks pass magnitude-based diagonal dominance: visual $11/16$, language $2/16$, and alignment $5/16$. The remaining $30/48$ failures match Proposition~\ref{prop:probe_entanglement}. Visual ruin is often magnitude-selective, while language and alignment interventions are much less selective. A damaged image can induce prior guessing, a corrupted question can alter binding, and a relation perturbation can be ignored when the answer already follows a prior. Hence, $(V,L,A)$ is a joint source signature rather than causal labels.

\paragraph{Signatures Diagnose Failure Families.}
Although the scores are entangled, their joint pattern is diagnostic. We observe from Table~\ref{tab:diagnosis_importance_main} that XGBoost improves from $0.78$ AUROC with scalar confidence to $0.95$ with $(V,L,A)$, and to $0.97$ with confidence added back. Other classifiers follow. Proposition~\ref{prop:diagnosis_not_abstention} formalizes this role separation: source signatures can carry failure-type information without serving as correctness-ranking scores. The gain is not only prevalence-driven, since alignment contributes $0.50$ of pooled XGBoost importance. Dataset-identity controls bound the claim. Adding $V+L+A$ improves raw-family Macro-F1 from $0.71$ to $0.78$, while the stricter outcome-family setting improves from $0.31$ to $0.35$. Fixed-dataset checks are strongest on HallusionBench and VizWiz, weaker on POPE, and negative on VSR. A blind audit gives the same direction: clear-source labels are mostly alignment ($71/107$), and $(V,L,A)$ improves clear-source AUROC over scalar confidence from $0.43$ to $0.60$.

\paragraph{Scalarization is a Wrong Target.}
The diagnostic result raises a decision question: \textit{Since source signatures predict failure type, can they be converted into a better abstention score}? Corollary~\ref{cor:no_source_complete_scalar_reliability} shows that a scalar abstention interface can be selective without identifying the failure source. We observe from Table~\ref{tab:decision_behavior_main} that weighted, geometric, and max-penalty scalarizations all underperform in AUROC. Qwen3-VL drops from $0.81$ scalar AUROC to $0.73$ for the best source-aware score. This does not certify scalar confidence as grounded. It shows that source-aware uncertainty should not be forced into the same scalar abstention interface. Proposition~\ref{prop:pairwise_inversion} formalizes the ranking risk: source penalties can reverse useful confidence orderings when penalty variation is not aligned with correctness, and near-saturated $L$ can flatten many examples.

\paragraph{Diagnosis-Triggered Routing.}
We test whether source signatures choose safer correction paths. Generic prompting applies one reasoning prompt to every example, while matched routing selects visual re-grounding, anti-prior prompting, or relation checking from normalized source dominance. We observe from Table~\ref{tab:decision_behavior_main} that matched routing is not a universal accuracy booster: it beats generic prompting in $10/16$ settings, with pooled accuracy $75.9\%$ versus $75.7\%$ for generic prompting and $76.6\%$ without intervention. Its value is clearer in break-rate control. On Qwen3-VL/VSR, matched routing avoids the generic accuracy drop from $87.4\%$ to $76.2\%$ and lowers breakage from $15.5\%$ to $2.7\%$, while maintaining $87.6\%$ accuracy. On Gemma 4/HallusionBench, it avoids the $68.2\%$ to $60.9\%$ generic drop and lowers breakage from $15.1\%$ to $4.9\%$. On LLaVA-Mistral/VizWiz, both interventions reduce accuracy, although matched routing lowers breakage from $21.4\%$ to $17.4\%$. This supports routing when generic correction risks damaging correct predictions. Since baseline accuracy exceeds $0.5$, Corollary~\ref{cor:break_rate_importance} gives larger weight to avoiding broken correct answers than to an equal-sized repair gain. Full supporting tables appear in Appendix Tables~\ref{tab:app_source_profiles_full}-\ref{tab:app_intervention_win_counts}.

==> emnlp2023-latex/Tables/App-Tab-Dataset-composition.tex <==
\begin{table*}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{lrrp{6.5cm}}
\toprule
\textbf{Dataset} & \textbf{Per-Model $N$} & \textbf{Pooled $N$} & \textbf{Failure-Family Counts Per Model} \\
\midrule
HallusionBench & 951 & 3804 & attribute=360, object hallucination=591 \\
POPE & 9000 & 36000 & object hallucination=9000 \\
VizWiz & 4319 & 17276 & answerability=1385, none=2934 \\
VSR & 340 & 1360 & spatial=340 \\
\bottomrule
\end{tabular}
}
\caption{Dataset composition used for pooled source-signature analyses.}
\label{tab:app_dataset_composition}
\end{table*}

==> emnlp2023-latex/Tables/Tab-Abstention-trap.tex <==
\begin{table}[t]
\centering
\scalebox{0.51}{
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Scalar AUROC} & \textbf{Best SA AUROC} & \textbf{Scalar Sel@60} & \textbf{Best SA Sel@60} \\
\midrule
Gemma 4 & 0.809 & 0.773 & 90.8\% & 88.3\% \\
LLaVA-Mistral & 0.836 & 0.806 & 91.9\% & 90.3\% \\
LLaVA-Vicuna & 0.828 & 0.778 & 90.8\% & 88.5\% \\
Qwen3-VL & 0.809 & 0.732 & 93.0\% & 89.9\% \\
\bottomrule
\end{tabular}
}
\caption{Aggregate abstention results. SA denotes the best source-aware confidence variant for each model.}
\label{tab:abstention_trap}
\end{table}

==> emnlp2023-latex/Tables/Tab-Datasets.tex <==
\begin{table}[t]
\centering
\scalebox{0.5}{
\begin{tabular}{lcll}
\toprule
\textbf{Dataset} & \textbf{Samples} & \textbf{Task Format} & \textbf{Primary Failure Mode} \\
\midrule
HallusionBench & 951 & Yes/No & Visual illusion and attribute hallucination \\
POPE & 9{,}000 & Yes/No & Object hallucination \\
VSR & 340 & True/False & Spatial and relation error \\
VizWiz-VQA & 4{,}319 & Open-ended VQA & Visual insufficiency and answerability failure \\
\bottomrule
\end{tabular}
}
\caption{Datasets used in the main evaluation. We use image-paired HallusionBench examples, all three POPE splits, the zero-shot VSR dev split, and the VizWiz validation split.}
\label{tab:datasets}
\end{table}

==> emnlp2023-latex/Tables/Tab-Decision-routing-summary.tex <==
\begin{table*}[t]
\centering
\scalebox{0.56}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Model / Setting} & \textbf{Scalar AUROC} & \textbf{Best SA AUROC} & \textbf{Scalar Sel@60} & \textbf{Best SA Sel@60} & \textbf{Matched Acc.} & \textbf{Break$_M$} \\
\midrule
Gemma 4 & 0.809 & 0.773 & 90.8\% & 88.3\% & -- & -- \\
LLaVA-Mistral & 0.836 & 0.806 & 91.9\% & 90.3\% & -- & -- \\
LLaVA-Vicuna & 0.828 & 0.778 & 90.8\% & 88.5\% & -- & -- \\
Qwen3-VL & 0.809 & 0.732 & 93.0\% & 89.9\% & -- & -- \\
\midrule
Pooled routing & -- & -- & -- & -- & 75.9\% & 3.9\% \\
Qwen3-VL/VSR & -- & -- & -- & -- & 87.6\% & 2.7\% \\
Gemma 4/HallusionBench & -- & -- & -- & -- & 68.9\% & -- \\
LLaVA-Mistral/HallusionBench & -- & -- & -- & -- & 53.8\% & -- \\
LLaVA-Vicuna/HallusionBench & -- & -- & -- & -- & 50.4\% & -- \\
\bottomrule
\end{tabular}
}
\caption{Abstention and routing summary. SA denotes the best source-aware confidence variant for each model. Matched Acc. and Break$_M$ denote matched-routing accuracy and break rate. Full generic and no-intervention comparisons appear in Appendix~\ref{app:intervention_routing}.}
\label{tab:decision_routing_summary}
\end{table*}


==> emnlp2023-latex/Tables/Tab-Entanglement-combined.tex <==
\begin{table}[t]
\centering
\scalebox{0.46}{
\begin{tabular}{lrrrc}
\toprule
\textbf{Intervention} & $\mathbf{\Delta V}$ & $\mathbf{\Delta L}$ & $\mathbf{\Delta A}$ & \textbf{Pass} \\
\midrule
Visual-ruined & -0.085 & +0.011 & -0.009 & 0/16 \\
Language-ruined & -0.047 & -0.086 & +0.175 & 2/16 \\
Alignment-ruined & -0.001 & +0.000 & +0.002 & 5/16 \\
\midrule
All checks & -- & -- & -- & 7/48 \\
\bottomrule
\end{tabular}
}
\caption{Interventional entanglement. The $\Delta$ columns show Qwen3-VL/HallusionBench. Pass counts summarize diagonal dominance over model-dataset settings.}
\label{tab:entanglement_combined}
\end{table}


==> emnlp2023-latex/Tables/Tab-Entanglement-matrix.tex <==
\begin{table}[t]
\centering
\scalebox{0.6}{
\begin{tabular}{lrrrl}
\toprule
\textbf{Intervention} & $\mathbf{\Delta V}$ & $\mathbf{\Delta L}$ & $\mathbf{\Delta A}$ & \textbf{Target} \\
\midrule
Visual-ruined & -0.085 & +0.011 & -0.009 & $V$ \\
Language-ruined & -0.047 & -0.086 & +0.175 & $L$ \\
Alignment-ruined & -0.001 & +0.000 & +0.002 & $A$ \\
\bottomrule
\end{tabular}
}
\caption{Interventional entanglement on Qwen3-VL/HallusionBench. Each entry is the change from the clean source score.}
\label{tab:entanglement_matrix}
\end{table}

==> emnlp2023-latex/Tables/Tab-Entanglement-summary.tex <==
\begin{table}[t]
\centering
\scalebox{0.6}{
\begin{tabular}{lccc}
\toprule
\textbf{Intervention} & \textbf{Pass} & \textbf{Fail} & \textbf{Pass Rate} \\
\midrule
Visual-ruined & 0 & 16 & 0.0\% \\
Language-ruined & 2 & 14 & 12.5\% \\
Alignment-ruined & 5 & 11 & 31.2\% \\
\midrule
All checks & 7 & 41 & 14.6\% \\
\bottomrule
\end{tabular}
}
\caption{Diagonal-dominance outcomes over $16$ model-dataset settings.}
\label{tab:entanglement_summary}
\end{table}

==> emnlp2023-latex/Tables/Tab-Failure-diagnosis.tex <==
\begin{table}[t]
\centering
\scalebox{0.6}{
\begin{tabular}{lccc}
\toprule
\textbf{Classifier} & \textbf{Scalar} & $\mathbf{V+L+A}$ & $\mathbf{V+L+A+\textbf{Scalar}}$ \\
\midrule
Logistic Regression & 0.752$\pm$0.002 & 0.828$\pm$0.003 & 0.873$\pm$0.002 \\
XGBoost & 0.781$\pm$0.002 & 0.954$\pm$0.002 & 0.971$\pm$0.001 \\
LightGBM & 0.780$\pm$0.002 & 0.953$\pm$0.002 & 0.968$\pm$0.002 \\
\bottomrule
\end{tabular}
}
\caption{Pooled failure-family diagnosis over $58{,}440$ samples. We report weighted AUROC across five failure families.}
\label{tab:failure_diagnosis}
\end{table}

==> emnlp2023-latex/Tables/Tab-Feature-importance.tex <==
\begin{table}[t]
\centering
\scalebox{0.6}{
\begin{tabular}{lcc}
\toprule
\textbf{Feature} & \textbf{XGBoost} & \textbf{LightGBM} \\
\midrule
$A$ & 0.504 & 0.360 \\
$L$ & 0.200 & 0.146 \\
Scalar confidence & 0.150 & 0.271 \\
$V$ & 0.147 & 0.222 \\
\bottomrule
\end{tabular}
}
\caption{Pooled feature importance for failure-family diagnosis.}
\label{tab:feature_importance}
\end{table}

==> emnlp2023-latex/Tables/Tab-Intervention-routing.tex <==
\begin{table}[t]
\centering
\scalebox{0.53}{
\begin{tabular}{lccccc}
\toprule
\textbf{Setting} & \textbf{No Interv.} & \textbf{Generic} & \textbf{Matched} & \textbf{Fix$_M$} & \textbf{Break$_M$} \\
\midrule
Pooled & 76.6\% & 75.7\% & 75.9\% & -- & 3.9\% \\
Qwen3-VL/VSR & 87.4\% & 76.2\% & 87.6\% & 20.9\% & 2.7\% \\
Gemma 4/HallusionBench & 68.2\% & 60.9\% & 68.9\% & 12.6\% & -- \\
LLaVA-Mistral/HallusionBench & 52.6\% & 50.9\% & 53.8\% & 12.0\% & -- \\
LLaVA-Vicuna/HallusionBench & 47.7\% & 47.9\% & 50.4\% & 13.3\% & -- \\
\bottomrule
\end{tabular}
}
\caption{Intervention routing results. Fix$_M$ and Break$_M$ denote the matched-policy fix and break rates.}
\label{tab:intervention_routing}
\end{table}

==> emnlp2023-latex/Tables/Tab-Method-costs.tex <==
\begin{table}[t]
\centering
\scalebox{0.6}{
\begin{tabular}{lcc}
\toprule
\textbf{Quantity} & \textbf{Probe} & \textbf{Forward Passes} \\
\midrule
Scalar confidence $c$ & Clean input & 1 \\
Visual score $V$ & Image perturbations & 4 \\
Image-removal confidence retention $L$ & Blank image & 1 \\
Alignment score $A$ & Grounding and relation probes & 1--2 \\
\midrule
\textbf{Total} & \textbf{All probes} & \textbf{7--8} \\
\bottomrule
\end{tabular}
}
\caption{Inference cost per example. The method uses controlled inference-time probes and does not require model retraining.}
\label{tab:method_cost}
\end{table}

==> emnlp2023-latex/Tables/Tab-Models.tex <==
\begin{table}[t]
\centering
\scalebox{0.45}{
\begin{tabular}{lll}
\toprule
\textbf{Model} & \textbf{Backbone Family} & \textbf{Role In Evaluation} \\
\midrule
Gemma 4 & Gemma-family MLLM & Compact recent MLLM setting \\
LLaVA-Mistral & LLaVA with Mistral backend & LLaVA-family model with Mistral language backbone \\
LLaVA-Vicuna & LLaVA with Vicuna backend & LLaVA-family model with Vicuna language backbone \\
Qwen3-VL & Qwen-family MLLM & Strong general-purpose vision-language model \\
\bottomrule
\end{tabular}
}
\caption{Model families used in the main evaluation. Full checkpoint names and hardware details are provided in Appendix~\ref{app:implementation_details}.}
\label{tab:models}
\end{table} 

==> emnlp2023-latex/Tables/Tab-Results-evidence-summary.tex <==
\begin{table}[t]
\centering
\scalebox{0.54}{
\begin{tabular}{lll}
\toprule
\textbf{Claim} & \textbf{Setting} & \textbf{Value} \\
\midrule
Entanglement & All checks & $7/48$ pass \\
Entanglement & Qwen3-VL/HB & $\Delta V=-0.085$, $\Delta L=-0.086$, $\Delta A=+0.175$ \\
Diagnosis & Logistic Reg. & $0.752 \rightarrow 0.828 \rightarrow 0.873$ \\
Diagnosis & XGBoost & $0.781 \rightarrow 0.954 \rightarrow 0.971$ \\
Diagnosis & LightGBM & $0.780 \rightarrow 0.953 \rightarrow 0.968$ \\
Importance & XGBoost & $A/L/c/V=0.504/0.200/0.150/0.147$ \\
Abstention & Qwen3-VL & $0.809$ scalar vs $0.732$ source-aware \\
Routing & Qwen3-VL/VSR & $87.4 \rightarrow 76.2 \rightarrow 87.6\%$; break $15.5 \rightarrow 2.7\%$ \\
\bottomrule
\end{tabular}
}
\caption{Compact evidence summary. Diagnosis arrows denote scalar $\rightarrow$ $(V,L,A)$ $\rightarrow$ $(V,L,A,c)$ AUROC. Routing arrows denote no intervention $\rightarrow$ generic prompting $\rightarrow$ matched routing. HB abbreviates HallusionBench.}
\label{tab:results_evidence_summary}
\end{table}


==> emnlp2023-latex/Tables/Tab-Source-signature-profile.tex <==
\begin{table}[t]
\centering
\scalebox{0.54}{
\begin{tabular}{llc}
\toprule
\textbf{Pattern} & \textbf{Slice} & \textbf{Value} \\
\midrule
Mean $L$ range & All model-dataset settings & 0.914--1.000 \\
LP match range & All model-dataset settings & 37.6--96.5\% \\
Highest $V$ range & VizWiz settings & 0.192--0.303 \\
Highest $A$ values & Gemma 4/VSR, Qwen3-VL/VSR & 0.675, 0.613 \\
Raw dominance & $L/A/V$ over $58{,}440$ samples & 58{,}287 / 151 / 2 \\
\bottomrule
\end{tabular}
}
\caption{Compact source-profile summary. LP Match denotes answer consistency between the original image and blank-image condition. The full model-dataset grid is provided in Appendix~\ref{app:full_source_profiles}.}
\label{tab:source_profiles}
\end{table}

